TTN: A Domain-Shift Aware Batch Normalization in Test-Time Adaptation

This paper proposes a novel batch normalization strategy for test-time adaptation. Recent test-time adaptation methods heavily rely on the modified batch normalization, i.e., transductive batch normalization (TBN), which calculates the mean and the variance from the current test batch rather than using the running mean and variance obtained from the source data, i.e., conventional batch normalization (CBN). Adopting TBN that employs test batch statistics mitigates the performance degradation caused by the domain shift. However, re-estimating normalization statistics using test data depends on impractical assumptions that a test batch should be large enough and be drawn from i.i.d. stream, and we observed that the previous methods with TBN show critical performance drop without the assumptions. In this paper, we identify that CBN and TBN are in a trade-off relationship and present a new test-time normalization (TTN) method that interpolates the statistics by adjusting the importance between CBN and TBN according to the domain-shift sensitivity of each BN layer. Our proposed TTN improves model robustness to shifted domains across a wide range of batch sizes and in various realistic evaluation scenarios. TTN is widely applicable to other test-time adaptation methods that rely on updating model parameters via backpropagation. We demonstrate that adopting TTN further improves their performance and achieves state-of-the-art performance in various standard benchmarks.

==> tables/cls_imbalance.tex <==
\begin{table}[h]{}
% \begin{minipage}[b]{70mm}
    \vspace{-0.3cm}
    \caption{\textbf{Adaptation on class imbalanced target domain.} 
    Error rate ($\downarrow$) averaged over 15 corruptions of CIFAR-10-C where test data is sorted in class label order and composed into test batches.}
    \vspace{-0.1cm}
    \centering
    \begin{adjustbox}{width=0.8\textwidth}
    \begin{tabular}{c||cccccc|c}
    \toprule
    
    \multirow{2}{*}{\textbf{Method}} &
    \multicolumn{6}{c|}{\textbf{Test batch size}} &
    \multirow{2}{*}{\textbf{Avg.}} \\
    
    \cmidrule{2-7}
    & 200 & 64 & 16 & 4 & 2& 1 & \\
    
    \midrule
    \midrule
    
    Source & 18.27 & 18.27 & 18.27 & 18.27 & 18.27 & 18.27 & 18.27\\
    \midrule
    TBN & 77.60 & 76.66 & 77.72 & 78.59 & 77.84 & 90.00 & 79.74 \\
    \rowcolor{Gray} \textbf{Ours (TTN)} & \textbf{35.75} & \textbf{35.13} & \textbf{34.92} & \textbf{32.51} & \textbf{28.60} & \textbf{17.99} & \textbf{30.82}\\
    
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \vspace{-0.0cm}
    \label{tab:class_imbalance}
% \end{minipage}
\end{table}

==> tables/mix_trg_tta.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table}[t]
% % \begin{minipage}{.5\linewidth}
% \caption{\textbf{Mixed domain adaptation on corruption benchmark.} 
% Error rate ($\downarrow$) of mixed domain with severity level 5 is reported for each test batch size.
% \textit{Optim.} denotes that (partial or entire) model parameters are updated in test-time.
% }
% \begin{subtable}[h]{\textwidth}
%     \caption{CIFAR-10-C (WRN-40-2)}
%     % \begin{center}
%     % \fontsize{7.8}{10pt}\selectfont
%     \centering
    
%     \begin{adjustbox}{width=0.9\textwidth}
%     \begin{tabular}{c|c|cccccc|c}
%     \toprule
    
%     & \multirow{2}{*}{\textbf{Method}} &
%     \multicolumn{6}{c|}{\textbf{Test batch size}} &
%     \multirow{2}{*}{\textbf{Avg.}}\\
    
%     \cmidrule{3-8}
%     & & 200 & 64 & 16 & 4 & 2 & 1& \\
    
%     \midrule
%     \midrule
    
%     & Source (CBN) & 18.27 & 18.27 & 18.27 & 18.27 & 18.27 & 18.27 & 18.27 \\
    
%     \midrule
    
%     \multirow{4}{*}{\rotatebox[origin=c]{90}{Optim.}} 
%     & TENT~\citep{wang2020tent} & 14.27 & 15.25 & 16.82 & 26.13 & 35.95 & 90.00 & 33.07\\
%     & \cellcolor{Gray} TENT+\textbf{TTN (Ours)} & \textbf{11.73} & \textbf{12.11} & \textbf{11.97} & \textbf{13.67} & \textbf{16.06} & \textbf{17.80} & \textbf{13.89}\\
    
%     \cmidrule{2-9}
%     % & \hs{SWR} & 10.81 & 14.39 & 21.36 & 34.80 & 64.61 & 90.08 & \textbf{39.34} \\
%     % & \hs{\cellcolor{Gray} SWR+\textbf{TTN (Ours)}} & 27.24 & \hs{73.79} & \hs{70.94} & \hs{67.70} & 68.67 & 65.01 & 62.23 \\
%     & SWR~\citep{choi2022improving} & 12.96 & 12.70 & 14.47 & 24.26 & 34.43 & 90.00 & 31.47\\
%     & {\cellcolor{Gray} SWR+\textbf{TTN (Ours)}} &\textbf{11.65} & \textbf{11.44} & \textbf{12.08} & \textbf{14.14} & \textbf{17.15} & \textbf{19.55} & \textbf{14.34}\\
    

%     \bottomrule
%     \end{tabular}
%     \end{adjustbox}
% \end{subtable}


% \begin{subtable}[h]{\textwidth}
%     \caption{CIFAR-100-C (WRN-40-2)}
%     % \begin{center}
%     % \fontsize{7.8}{10pt}\selectfont
%     \centering
    
%     \begin{adjustbox}{width=0.9\textwidth}
%     \begin{tabular}{c |c|cccccc|c}
%     \toprule

%     & \multirow{2}{*}{\textbf{Method}} &
%     \multicolumn{6}{c|}{\textbf{Test batch size}} 
%     & \multirow{2}{*}{\textbf{Avg.}} \\
    
%     \cmidrule{3-8}
%     & & 200 & 64 & 16 & 4 & 2& 1\\
    
%     \midrule
%     \midrule
    
%     & Source (CBN) & 46.75 & 46.75 & 46.75 & 46.75 & 46.75 & 46.75 & 46.75 \\
    
%     \midrule
    
%     \multirow{4}{*}{\rotatebox[origin=c]{90}{Optim.}} 
%     & TENT~\citep{wang2020tent} & 36.86 & 40.28 & 43.47 & 59.52 & 80.29 & 98.97 & 59.90 \\
%     & \cellcolor{Gray} TENT+\textbf{TTN (Ours)}  & \textbf{35.90} & \textbf{36.17} & \textbf{36.39} & \textbf{41.86} & \textbf{46.95} & \textbf{59.08} & \textbf{42.73}\\ 
    
%     \cmidrule{2-9}
%     & SWR~\citep{choi2022improving} & 36.60 & 36.99 & 40.18 & 57.76 & 78.86 & 99.07& 58.24\\
%     & \cellcolor{Gray} SWR+\textbf{TTN (Ours)}& \textbf{35.67} & \textbf{35.59} & \textbf{36.90} & \textbf{42.20} & \textbf{48.60} & \textbf{69.29} & \textbf{44.71}\\
    
%     \bottomrule
%     \end{tabular}
%     \end{adjustbox}
% \end{subtable}

% \label{tab:mix_trg_tta}
% \end{table}
% % \end{minipage}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
% \begin{minipage}{.5\linewidth}
\caption{\textbf{Mixed domain adaptation on corruption benchmark.} 
Error rate ($\downarrow$) of mixed domain with severity level 5 is reported for each test batch size.
% \textit{Optim.} denotes that (partial or entire) model parameters are updated in test-time.
% Error rate ($\downarrow$) on \hs{mixed domain with 15 corruption types with severity level 5} is reported for each test batch size.
}
% \begin{subtable}[h]{\textwidth}
%     \caption{CIFAR-10-C (WRN-40-2)}
    % \begin{center}
    % \fontsize{7.8}{10pt}\selectfont
    \centering
    \vspace{-0.1in}
    \begin{adjustbox}{width=1.0\textwidth}
    \setlength\tabcolsep{3pt}
    \begin{tabular}{c|c||cccccc|c||cccccc|c}
    % \toprule
    
    % & &
    % \multicolumn{7}{c||}{\textbf{CIFAR-10-C}} 
    % & \multicolumn{7}{c}{\textbf{CIFAR-100-C}} \\
    
    % \midrule
    
    % & \multirow{2}{*}{\textbf{Method}} &
    % \multicolumn{6}{c|}{\textbf{Test batch size}} &
    % \multirow{2}{*}{\textbf{Avg.}} 
    % & \multicolumn{6}{c|}{\textbf{Test batch size}} &
    % \multirow{2}{*}{\textbf{Avg.}}\\
    
    % \cmidrule{3-8}\cmidrule{10-15}
    % & & 200 & 64 & 16 & 4 & 2 & 1& 
    % & 200 & 64 & 16 & 4 & 2 & 1& \\
    
    \toprule
     \multicolumn{2}{c||}{} & \multicolumn{7}{c||}{\textbf{CIFAR-10-C}} &
    \multicolumn{7}{c}{\textbf{CIFAR-100-C}} \\
    
    % \cmidrule{3-16}
    % \toprule
    
     \multicolumn{2}{c||}{\textbf{Method}} & 200 & 64 & 16 & 4 & 2& 1 & \textbf{Avg.}
    & 200 & 64 & 16 & 4 & 2& 1 & \textbf{Avg.} \\
    
    \midrule
    \midrule
    
    & Source & 18.27 & 18.27 & 18.27 & 18.27 & 18.27 & 18.27 & 18.27 
    & 46.75 & 46.75 & 46.75 & 46.75 & 46.75 & 46.75 & 46.75 \\
    
    \midrule
    
    & \cellcolor{Gray} \textbf{Ours (TTN)} &  \cellcolor{Gray}\textbf{11.67} &  \cellcolor{Gray}\textbf{11.80} & \cellcolor{Gray} \textbf{12.13} & \cellcolor{Gray} \textbf{13.93} & \cellcolor{Gray}\textbf{15.83} &  \cellcolor{Gray}\textbf{17.99} & \cellcolor{Gray}\textbf{13.89}
    &  \cellcolor{Gray}\textbf{35.58} &  \cellcolor{Gray}\textbf{35.84} &  \cellcolor{Gray}\textbf{36.73} &  \cellcolor{Gray}\textbf{41.08} &  \cellcolor{Gray}\textbf{46.67} &  \cellcolor{Gray}\textbf{57.71} & \cellcolor{Gray}\textbf{42.27}\\ 
    
    \midrule
    
    \multirow{4}{*}{\rotatebox[origin=c]{90}{Optim.}} 
    & TENT & 14.27 & 15.25 & 16.82 & 26.13 & 35.95 & 90.00 & 33.07
    & 36.86 & 40.28 & 43.47 & 59.52 & 80.29 & 98.97 & 59.90 \\
    
    & \cellcolor{Gray} +\textbf{Ours (TTN)} & \cellcolor{Gray}\textbf{11.73} & \cellcolor{Gray}\textbf{12.11} & \cellcolor{Gray}\textbf{11.97} & \cellcolor{Gray}\textbf{13.67} & \cellcolor{Gray}\textbf{16.06} & \cellcolor{Gray}\textbf{17.80} & \cellcolor{Gray}\textbf{13.89}
    & \cellcolor{Gray}\textbf{35.90} & \cellcolor{Gray}\textbf{36.17} & \cellcolor{Gray}\textbf{36.39} & \cellcolor{Gray}\textbf{41.86} & \cellcolor{Gray}\textbf{46.95} & \cellcolor{Gray}\textbf{59.08} & \cellcolor{Gray}\textbf{42.73}\\ 
    
    \cmidrule{2-16}
    & SWR & 12.96 & 12.70 & 14.47 & 24.26 & 34.43 & 90.00 & 31.47
    & 36.60 & 36.99 & 40.18 & 57.76 & 78.86 & 99.07& 58.24\\
    
    & {\cellcolor{Gray} +\textbf{Ours (TTN)}} &\cellcolor{Gray}\textbf{11.65} &\cellcolor{Gray} \textbf{11.44} &\cellcolor{Gray} \textbf{12.08} & \cellcolor{Gray}\textbf{14.14} & \cellcolor{Gray}\textbf{17.15} & \cellcolor{Gray}\textbf{19.55} & \cellcolor{Gray}\textbf{14.34}
    & \cellcolor{Gray}\textbf{35.67} & \cellcolor{Gray}\textbf{35.59} & \cellcolor{Gray}\textbf{36.90} & \cellcolor{Gray} \textbf{42.20} & \cellcolor{Gray}\textbf{48.60} &\cellcolor{Gray} \textbf{69.29} & \cellcolor{Gray}\textbf{44.71}\\

    \bottomrule
    \end{tabular}
    \end{adjustbox}
% \end{subtable}


% \begin{subtable}[h]{\textwidth}
%     \caption{CIFAR-100-C (WRN-40-2)}
%     % \begin{center}
%     % \fontsize{7.8}{10pt}\selectfont
%     \centering
    
%     \begin{adjustbox}{width=0.9\textwidth}
%     \begin{tabular}{c |c|cccccc|c}
%     \toprule

%     & \multirow{2}{*}{\textbf{Method}} &
%     \multicolumn{6}{c|}{\textbf{Test batch size}} 
%     & \multirow{2}{*}{\textbf{Avg.}} \\
    
%     \cmidrule{3-8}
%     & & 200 & 64 & 16 & 4 & 2& 1\\
    
%     \midrule
%     \midrule
    
%     & Source & 46.75 & 46.75 & 46.75 & 46.75 & 46.75 & 46.75 & 46.75 \\
    
%     \midrule
    
%     \multirow{4}{*}{\rotatebox[origin=c]{90}{Optim.}} 
%     & TENT & 36.86 & 40.28 & 43.47 & 59.52 & 80.29 & 98.97 & 59.90 \\
%     & \cellcolor{Gray} +\textbf{Ours (TTN)}  & \textbf{35.90} & \textbf{36.17} & \textbf{36.39} & \textbf{41.86} & \textbf{46.95} & \textbf{59.08} & \textbf{42.73}\\ 
    
%     \cmidrule{2-9}
%     & SWR & 36.60 & 36.99 & 40.18 & 57.76 & 78.86 & 99.07& 58.24\\
%     & \cellcolor{Gray} +\textbf{Ours (TTN)}& \textbf{35.67} & \textbf{35.59} & \textbf{36.90} & \textbf{42.20} & \textbf{48.60} & \textbf{69.29} & \textbf{44.71}\\
    
%     \bottomrule
%     \end{tabular}
%     \end{adjustbox}
% \end{subtable}

\label{tab:mix_trg_tta_old}
\end{table}
% \end{minipage}

==> tables/src_tta.tex <==
% \begin{table}[t]{}
%     \caption{\textbf{Adaptation on source domain test data}.
%     Error rate ($\downarrow$) of source domain test data (CIFAR-10) is reported with backbone WRN-40~\citep{zagoruyko2016wide,hendrycks2019augmix}.
%     Evaluated in single domain adaptation scenario.
%     \textit{Norm} denotes that only standardization statistics are updated in test-time, while model parameters are frozen.
%     \textit{Optim.} denotes that (partial or entire) model parameters are updated in test-time.}
%     \centering
%     \begin{adjustbox}{width=0.9\textwidth}
%     \begin{tabular}{c |c|cccccc|c}
%     \toprule
    
%     & \multirow{2}{*}{\textbf{Method}} &
%     \multicolumn{6}{c|}{\textbf{Test batch size}} &
%     \multirow{2}{*}{\textbf{Avg.}} \\
    
%     \cmidrule{3-8}
%     & & 200 & 64 & 16 & 4 & 2 & 1& \\
    
%     \midrule
%     \midrule
    
%     & Source (CBN) & 4.92 & 4.92 & 4.92 & 4.92 & 4.92 & 4.92 & 4.92\\
%     \midrule
    
%     \multirow{2}{*}{\rotatebox[origin=c]{90}{Norm}}
%     & TBN~\citep{schneider2020improving} & 6.41 & 6.60 & 8.64 & 17.65 & 26.08 & 90.00 & 25.90 \\
    
%     & \cellcolor{Gray} \textbf{TTN (Ours)} & \textbf{4.88} & \textbf{5.11} & \textbf{5.35} & \textbf{7.27} & \textbf{9.45} & \textbf{9.96} & \textbf{7.00} \\
    
%     \midrule
%     \multirow{4}{*}{\rotatebox[origin=c]{90}{Optim.}} 
%     & TENT~\citep{wang2020tent} & 6.15 & 6.45 & 	8.61 & 	17.61 & 26.20 & 90.00 & 32.2\\
%     & \cellcolor{Gray} TENT+\textbf{TTN (Ours)} & \textbf{4.93} & \textbf{5.11} & \textbf{5.32}  & \textbf{7.22}  & \textbf{9.38} & \textbf{10.21} & \textbf{7.02} \\
    
%     \cmidrule{2-9}
%     % & \hs{SWR~\citep{choi2022improving}} & 5.46 & 6.44	 & 8.89 & 19.55 & 30.86 & 90.05 & 30.96\\ 
%     % & \cellcolor{Gray} SWR+\textbf{TTN (Ours)} & \textbf{5.39} & \textbf{6.89}  & \textbf{7.54}  & \textbf{11.00} & \textbf{13.87} & \textbf{19.75} & \textbf{10.74} \\
%     & SWR~\citep{choi2022improving} &5.63 & 6.01 & 8.25 & 17.49 & 26.32 &90.00 & 25.62\\ 
%     & \cellcolor{Gray} SWR+\textbf{TTN (Ours)} & \textbf{4.79} & \textbf{5.02} & \textbf{5.51} & \textbf{6.68} & \textbf{7.91} & \textbf{9.34} & \textbf{6.54} \\
    
%     \bottomrule
%     \end{tabular}
%     \end{adjustbox}
    
%     \label{tab:src_tta}
% \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[h]{}
% \begin{minipage}[b]{70mm}
    \vspace{-0.05in}
    \caption{\textbf{Adaptation on source domain test set.} 
    Error rate ($\downarrow$) on test split of CIFAR-10 using WideResNet-40-2 is reported for each test batch size.
    }
    \vspace{-0.05in}
    % Error rate ($\downarrow$) of source domain test data (CIFAR-10) is reported with backbone WRN-40~\citep{zagoruyko2016wide,hendrycks2019augmix}.
    % Evaluated in single domain adaptation scenario.
    % \textit{Norm} denotes that only standardization statistics are updated in test-time, while model parameters are frozen.
    % \textit{Optim.} denotes that (partial or entire) model parameters are updated in test-time.}
    \centering
    \begin{adjustbox}{width=0.8\textwidth}
    % \setlength\tabcolsep{3pt}
    \begin{tabular}{c |c||cccccc|c}
    \toprule
    
    & \multirow{2}{*}{\textbf{Method}} &
    \multicolumn{6}{c|}{\textbf{Test batch size}} &
    \multirow{2}{*}{\textbf{Avg.}} \\
    
    \cmidrule{3-8}
    & & 200 & 64 & 16 & 4 & 2 & 1& \\
    
    \midrule
    \midrule
    
    & Source & 4.92 & 4.92 & 4.92 & 4.92 & 4.92 & 4.92 & 4.92\\
    \midrule
    
    \multirow{2}{*}{\rotatebox[origin=c]{90}{Norm}}
    & TBN & 6.41 & 6.60 & 8.64 & 17.65 & 26.08 & 90.00 & 25.90 \\
    
    & \cellcolor{Gray} \textbf{Ours (TTN)} & \cellcolor{Gray}\textbf{4.88} & \cellcolor{Gray}\textbf{5.11} & \cellcolor{Gray}\textbf{5.35} & \cellcolor{Gray}\textbf{7.27} & \cellcolor{Gray}\textbf{9.45} &\cellcolor{Gray} \textbf{9.96} & \cellcolor{Gray}\textbf{7.00} \\
    
    \midrule
    \multirow{4}{*}{\rotatebox[origin=c]{90}{Optim.}} 
    & TENT& 6.15 & 6.45 & 	8.61 & 	17.61 & 26.20 & 90.00 & 32.2\\
    & \cellcolor{Gray} +\textbf{Ours (TTN)} & \cellcolor{Gray}\textbf{4.93} & \cellcolor{Gray}\textbf{5.11} & \cellcolor{Gray}\textbf{5.32}  & \cellcolor{Gray}\textbf{7.22}  & \cellcolor{Gray}\textbf{9.38} & \cellcolor{Gray}\textbf{10.21} & \cellcolor{Gray}\textbf{7.02} \\
    
    \cmidrule{2-9}
    % & \hs{SWR~\citep{choi2022improving}} & 5.46 & 6.44	 & 8.89 & 19.55 & 30.86 & 90.05 & 30.96\\ 
    % & \cellcolor{Gray} SWR+\textbf{TTN (Ours)} & \textbf{5.39} & \textbf{6.89}  & \textbf{7.54}  & \textbf{11.00} & \textbf{13.87} & \textbf{19.75} & \textbf{10.74} \\
    & SWR &5.63 & 6.01 & 8.25 & 17.49 & 26.32 &90.00 & 25.62\\ 
    & \cellcolor{Gray} +\textbf{Ours (TTN)} & \cellcolor{Gray}\textbf{4.79} & \cellcolor{Gray}\textbf{5.02} & \cellcolor{Gray}\textbf{5.51} & \cellcolor{Gray}\textbf{6.68} & \cellcolor{Gray}\textbf{7.91} & \cellcolor{Gray}\textbf{9.34} & \cellcolor{Gray}\textbf{6.54} \\
    
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \vspace{-0.25cm}
    \label{tab:src_tta}
% \end{minipage}
\end{table}

% %%%%%%%%%%%%%%
% \begin{table}[h]
% \begin{minipage}[b]{80mm}
% \begin{tabular}{|c|l||r|r||r|r|}
% %//first table goes here
% \end{tabular}
%     \caption{some caption for first table} 
% \end{minipage}

% \begin{minipage}[b]{80mm}
% \begin{tabular}{|c|l||r|r||r|r|}
% %//second table goes here
% \end{tabular}
%     \caption{some caption for second table} 
% \end{minipage}

%  \end{table}

==> tables/sup_aug_ablation.tex <==
\begin{table}[ht]
    \caption{\textbf{Results of each corruption (CIFAR-10-C)}}
    \centering
    \begin{adjustbox}{width=1.0\textwidth}
    \begin{tabular}{c|c|ccccccccccccccc|c}
        
        \toprule
        \multicolumn{2}{c|}{Augmentation} & \multicolumn{15}{c|}{\textbf{Augmentation type in post-train}} & \\
        \midrule
        Obtaining prior & Optimizing alpha & gauss. & shot & impulse & defocus & glass & motion & zoom & snow & frost & fog & brightness & contrast & elastic & pixel. & jpeg. & Avg. \\
        \midrule
        Abalation & Fixed & 11.35&	11.41&	11.25&	11.66&	11.37&	11.65&	11.75&	11.64&	11.70&	11.78&	12.29&	11.87&	11.55&	11.47&	12.33& 11.74 \\
        Fixed & Ablation & 11.61&	11.61&	11.61&	11.92&	11.62&	11.81&	11.80&	11.83&	11.73&	11.69&	12.29&	11.60&	11.72&	11.49&	11.79& 11.67 \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    
    \label{appendix:tab:augmentation ablation}
    \vspace{-0.2cm}
\end{table}



==> tables/sup_cifar100_r50.tex <==
\begin{table}[ht]
    \caption{CIFAR-100-C (Resnet-50)}
    % \begin{center}
    % \fontsize{7.8}{10pt}\selectfont
    \centering
    
    \begin{adjustbox}{width=0.9\textwidth}
    \begin{tabular}{cc|cc|cc|cc|cc}
    \toprule
    
    \multicolumn{2}{c|}{\multirow{3}{*}{\textbf{Method}}} &
    \multicolumn{8}{c}{\textbf{Test batch size}} \\
    
    \cmidrule{3-10}
    & & \multicolumn{2}{c|}{200} & \multicolumn{2}{c|}{64} & \multicolumn{2}{c|}{16} & \multicolumn{2}{c}{4}\\
    
    \cmidrule{3-10}
    & & Single & Cont. & Single & Cont. & Single & Cont. & Single & Cont. \\
    
    \midrule
    \midrule
    
    & Soruce (CBN) & \multicolumn{2}{c|}{60.35} & \multicolumn{2}{c|}{60.35} & \multicolumn{2}{c|}{60.35} & \multicolumn{2}{c|}{60.35} \\

    
    \midrule
    
    \multirow{2}{*}{\rotatebox[origin=c]{90}{BN} }
    & TBN & \multicolumn{2}{c|}{43.68} & \multicolumn{2}{c|}{44.46} & \multicolumn{2}{c|}{47.69} & \multicolumn{2}{c}{61.11} \\
    & \cellcolor{Gray} \textbf{TTN} & \multicolumn{2}{c|}{\textbf{43.37}} & \multicolumn{2}{c|}{\textbf{43.81}} & \multicolumn{2}{c|}{\textbf{45.47}} & \multicolumn{2}{c}{{52.06}}\\ 
    
    \midrule
    \multirow{4}{*}{\rotatebox[origin=c]{90}{Parameters}}

    & TENT & 39.36	& 39.74	& 41.83	& 41.86	& 46.04	& 45.59	& 60.39	& 59.78 \\
    & \cellcolor{Gray} TENT+\textbf{TTN} & 39.08	& 40.15	& 40.79	& 41.27	& 44.01	& 43.50	& 52.64	& 51.99 \\
    & SWR & 38.49	& 35.61	& 75.28	& 41.34	& 88.40	& 72.59	& 93.68	& 97.52 \\
    & \cellcolor{Gray} TENT+\textbf{TTN}& 33.30	& 33.06	& 74.49	& 35.04	& 86.58	& 47.54	& 92.19	& 81.54 \\



    \bottomrule
    \end{tabular}
    \end{adjustbox}
    % \end{center}
    
    \label{tab:tab_cifar100_r50}
\end{table}

==> tables/sup_cifar10_r50.tex <==
\begin{table}[ht]
    \caption{CIFAR-10-C (Resnet-50)}
    % \begin{center}
    % \fontsize{7.8}{10pt}\selectfont
    \centering
    
    \begin{adjustbox}{width=0.9\textwidth}
    \begin{tabular}{cc|cc|cc|cc|cc}
    \toprule
    
    \multicolumn{2}{c|}{\multirow{3}{*}{\textbf{Method}}} &
    \multicolumn{8}{c}{\textbf{Test batch size}} \\
    
    \cmidrule{3-10}
    & & \multicolumn{2}{c|}{200} & \multicolumn{2}{c|}{64} & \multicolumn{2}{c|}{16} & \multicolumn{2}{c}{4}\\
    
    \cmidrule{3-10}
    & & Single & Cont. & Single & Cont. & Single & Cont. & Single & Cont. \\
    
    \midrule
    \midrule
    
    & Soruce (CBN) & \multicolumn{2}{c|}{29.14} & \multicolumn{2}{c|}{29.14} & \multicolumn{2}{c|}{29.14} & \multicolumn{2}{c}{29.14}\\

    
    \midrule
    
    \multirow{2}{*}{\rotatebox[origin=c]{90}{BN}} 
    & TBN & \multicolumn{2}{c|}{16.01} & \multicolumn{2}{c|}{16.52} & \multicolumn{2}{c|}{18.67} & \multicolumn{2}{c}{26.37} \\
    % & $\alpha$-BN & \multicolumn{2}{c|}{14.17} & \multicolumn{2}{c|}{14.67} & \multicolumn{2}{c|}{16.57} & \multicolumn{2}{c}{24.93}\\
    % & MixNormBN & \multicolumn{2}{c|}{18.52} & \multicolumn{2}{c|}{19.43} & \multicolumn{2}{c|}{20.19} & \multicolumn{2}{c}{\textbf{22.47} ($B$=5)} \\
    & \cellcolor{Gray} \textbf{TTN} & \multicolumn{2}{c|}{\textbf{15.85}} & \multicolumn{2}{c|}{\textbf{16.08}} & \multicolumn{2}{c|}{\textbf{16.90}} & \multicolumn{2}{c}{{20.49}}\\ 
    
    \midrule
    \multirow{4}{*}{\rotatebox[origin=c]{90}{Parameters}}
     
    & TENT & 14.21 & 14.34	& 15.61	& 15.58	& 18.18	& 17.89	& 26.45	& 26.17 \\
    & \cellcolor{Gray} TENT+\textbf{TTN} & 14.65 & 15.44	& 15.29	& 15.24	& 16.76	& 16.42	& 21.90	& 20.31 \\
    \cmidrule{2-10}
    & SWR & 12.96 & 13.92	& 37.67	& 25.37	& 52.94	& 58.96	& 67.70	& 75.93 \\
    & \cellcolor{Gray} TENT+\textbf{TTN} & 12.67	& 14.86	& 34.97	& 21.13	& 48.14	& 25.91	& 62.82	& 32.73 \\




    \bottomrule
    \end{tabular}
    \end{adjustbox}
    % \end{center}
    
    \label{tab:tab_cifar10_r50}
\end{table}

==> tables/sup_cifar10_w28.tex <==
\begin{table}[ht]
    \caption{CIFAR-10-C (WRN-28)}
    % \begin{center}
    % \fontsize{7.8}{10pt}\selectfont
    \centering
    
    \begin{adjustbox}{width=0.9\textwidth}
    \begin{tabular}{cc|cc|cc|cc|cc}
    \toprule
    
    \multicolumn{2}{c|}{\multirow{3}{*}{\textbf{Method}}} &
    \multicolumn{8}{c}{\textbf{Test batch size}} \\
    
    \cmidrule{3-10}
    & & \multicolumn{2}{c|}{200} & \multicolumn{2}{c|}{64} & \multicolumn{2}{c|}{16} & \multicolumn{2}{c}{4}\\
    
    \cmidrule{3-10}
    & & Single & Cont. & Single & Cont. & Single & Cont. & Single & Cont. \\
    
    \midrule
    \midrule
    
    & Soruce (CBN) & \multicolumn{2}{c|}{43.51} & \multicolumn{2}{c|}{43.51} & \multicolumn{2}{c|}{43.51} & \multicolumn{2}{c}{43.51} \\

    
    \midrule
    
    \multirow{2}{*}{\rotatebox[origin=c]{90}{BN} }
    & TBN & \multicolumn{2}{c|}{20.43} & \multicolumn{2}{c|}{20.93} & \multicolumn{2}{c|}{22.93} & \multicolumn{2}{c}{31.62} \\
    % & $\alpha$-BN & \multicolumn{2}{c|}{14.17} & \multicolumn{2}{c|}{14.67} & \multicolumn{2}{c|}{16.57} & \multicolumn{2}{c}{24.93}\\
    & MixNormBN & \multicolumn{2}{c|}{18.52} & \multicolumn{2}{c|}{19.43} & \multicolumn{2}{c|}{20.19} & \multicolumn{2}{c}{\textbf{22.47} ($B$=5)} \\
    & \cellcolor{Gray} \textbf{TTN} & \multicolumn{2}{c|}{\textbf{20.25}} & \multicolumn{2}{c|}{\textbf{20.52}} & \multicolumn{2}{c|}{\textbf{21.30}} & \multicolumn{2}{c}{{25.00}}\\ 
    
    \midrule
    \multirow{6}{*}{\rotatebox[origin=c]{90}{Parameters}}
    & TENT & 18.58 & 18.85 & 20.13 & 20.08 & 22.3 & 24.19 & 31.81 & 31.4 \\
    & \cellcolor{Gray} TENT+\textbf{TTN} &20.99 & 19.9 & 21.81 & 20.1 & 24.43 & 21.16 & 30.1 & 26.26 \\
    \cmidrule{2-10}
    & SWR &15.69 & 15.43 & 80.7 & 67.64 & 90.77 & 86.44 & 87.52 & 89.79\\
    & \cellcolor{Gray} SWR+\textbf{TTN} & 15.94 & 14.88 & 79.01 & 32.91 & 84.73 & 54.38 & 87.83 & 74.97\\
    \cmidrule{2-10}
    & CoTTA & - & 16.02(16.49) & - & 17.55 & - & 32.6 & - & 82.36\\
     & \cellcolor{Gray} CoTTA + \textbf{TTN} & - & 27.34 & - & 30.46 & - & 44.84 & - & 84.3\\



    \bottomrule
    \end{tabular}
    \end{adjustbox}
    % \end{center}
    
    \label{tab:tab_cifar10_w28}
\end{table}

==> tables/sup_evlv_trg_tta_swr_prev.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h]
\caption{\textbf{Continual adaptation on corruption benchmark.} 
Error rate ($\downarrow$) averaged over 15 corruption types with severity level 5 is reported for each test batch size.
Original version of SWR suffer from .
% \textit{Optim.} denotes that (partial or entire) model parameters are updated in test-time.
% {SWR $\theta_{prev}$}
}
\begin{subtable}[h]{\textwidth}
    \caption{CIFAR-10-C (WRN-40-2)}
    % \begin{center}
    % \fontsize{7.8}{10pt}\selectfont
    \centering
    
    \begin{adjustbox}{width=0.8\textwidth}
    \begin{tabular}{c|c|cccccc|c}
    \toprule
    
    & \multirow{2}{*}{\textbf{Method}} &
    \multicolumn{6}{c|}{\textbf{Test batch size}} &
    \multirow{2}{*}{\textbf{Avg.}}\\
    
    \cmidrule{3-8}
    & & 200 & 64 & 16 & 4 & 2 & 1& \\
    
    \midrule
    \midrule

    
    % \multirow{2}{*}{\rotatebox[origin=c]{90}{Optim.}} 
   
    % \cmidrule{2-9}
    & {SWR} & 10.81 & 14.39 & 21.36 & 34.80 & 64.61 & 90.08 & {39.34} \\
    & {\cellcolor{Gray} SWR+\textbf{TTN (Ours)}} & 27.24 & {73.79} & {70.94} & {67.70} & 68.67 & 65.01 & 62.23 \\
    % & SWR~\citep{choi2022improving} &11.04 & 11.53 & 13.90 & 23.99 & 34.02 &90.00 & 30.75 \\
    % & \cellcolor{Gray} SWR+\textbf{TTN (Ours)} & \textbf{10.09} & \textbf{10.51} & \textbf{11.28} & \textbf{14.29} & \textbf{16.67} & \textbf{84.12} & \textbf{24.49}\\
    
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    % \end{center}
    
    % \label{tab:c10_w40_evlv}
\end{subtable}


\begin{subtable}[h]{\textwidth}
    \vspace{0.1cm}
    \caption{CIFAR-100-C (WRN-40-2)}
    % \begin{center}
    % \fontsize{7.8}{10pt}\selectfont
    \centering
    
    \begin{adjustbox}{width=0.8\textwidth}
    \begin{tabular}{c |c|cccccc|c}
    \toprule
    
    % \textbf{Dataset} & \multicolumn{2}{c|} {CIFAR-100-C} &
    % \textbf{Backbone} & \multicolumn{2}{c} {WRN-40-2} \\
    % \midrule
    
    % \multirow{2}{*}{\textbf{Eval.}} &
    & \multirow{2}{*}{\textbf{Method}} &
    \multicolumn{6}{c|}{\textbf{Test batch size}} 
    & \multirow{2}{*}{\textbf{Avg.}} \\
    
    \cmidrule{3-8}
    & & 200 & 64 & 16 & 4 & 2& 1\\
    
    \midrule
    \midrule
    
    % & Source (CBN) & 46.75 & 46.75 & 46.75 & 46.75 & 46.75 & 46.75 & 46.75 \\
    
    % \midrule
    
    % \multirow{2}{*}{\rotatebox[origin=c]{90}{Optim.}} 
    % & TENT~\citep{wang2020tent} & \textbf{36.11} & 37.90 & 43.78 & 58.71 & 81.76 & 99.04 & 59.55 \\
    % & \cellcolor{Gray} TENT+\textbf{TTN} & 43.50 & \textbf{37.60} & \textbf{38.28} & \textbf{44.60} & \textbf{54.29} & \textbf{80.63} & \textbf{49.82} \\ 
    
    % \cmidrule{2-9}
    & SWR & 34.53 & 39.70 & 51.08 & 71.14 & 87.07 & 98.92 & 63.74\\
    & \cellcolor{Gray} {SWR+\textbf{TTN (Ours)}} & 76.41 & 90.85 & 87.26 & 77.85 & 82.42 & 86.85 &83.60\\
    
    % & SWR~\citep{choi2022improving}& 34.16 & 35.79 & 40.71 & 58.15 & 80.55 & 99.03 & 62.56\\
    % & \cellcolor{Gray} SWR+\textbf{TTN (Ours)} & \textbf{33.09} & \textbf{34.07} & \textbf{36.15} & \textbf{42.41} & \textbf{53.63} & \textbf{93.08} & \textbf{48.74} \\

    
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    
\end{subtable}
\label{tab:sup_evlv_trg_tta_swr}
\end{table}
